Virtual Correspondence: Humans as a Cue for Extreme-View Geometry

Recovering the spatial layout of the cameras and the geometry of the scene from extreme-view images is a longstanding challenge in computer vision. Prevailing 3D reconstruction algorithms often adopt the image matching paradigm and presume that a portion of the scene is co-visible across images, yielding poor performance when there is little overlap among inputs. In contrast, humans can associate visible parts in one image to the corresponding invisible components in another image via prior knowledge of the shapes. Inspired by this fact, we present a novel concept called virtual correspondences (VCs). VCs are a pair of pixels from two images whose camera rays intersect in 3D. Similar to classic correspondences, VCs conform with epipolar geometry; unlike classic correspondences, VCs do not need to be co-visible across views. Therefore VCs can be established and exploited even if images do not overlap. We introduce a method to find virtual correspondences based on humans in the scene. We showcase how VCs can be seamlessly integrated with classic bundle adjustment to recover camera poses across extreme views. Experiments show that our method significantly outperforms state-of-the-art camera pose estimation methods in challenging scenarios and is comparable in the traditional densely captured setup. Our approach also unleashes the potential of multiple downstream tasks such as scene reconstruction from multi-view stereo and novel view synthesis in extreme-view scenarios.

==> background.tex <==
\section{Preliminaries: Structure {from} Motion}
\sfm concerns the problem of recovering 3D structure of the scene as well as camera \slwang{poses} from a set of unordered images. 
While various forms of \sfm have been proposed in the past two decades, 
at the heart of these methods lie two key operations~\cite{hartleymultiple}: {correspondence estimation} and {bundle adjustment}. 
In this section, we briefly review the two concepts.
For simplicity, we assume there are only two cameras, but these concepts can be trivially extended to multi-camera setup.



\subsection{Correspondence Estimation}
\label{sec:correspondences}
We first define correspondences.
Let $\cI_1$, $\cI_2 \in \mathbb{R}^{H\times W \times 3}$  be the images of the same scene captured at different viewpoints and $\bp_{1}$, $\bp_{2} \in \mathbb{R}^{2}$ be their respective 2D pixel coordinates. We say the $i$-th pixel in the first image and the $j$-th pixel in the second image, $(\bp_{1, i}, \bp_{2, j})$, are \emph{correspondences} {if} they describe the same 3D point $\bX\in\mathbb{R}^3$ in the scene. 

To be more formal, let $\bK_1, \bK_2 \in \mathbb{R}^{3\times 3}$ be the camera intrinsics and $[\bR_1, \bt_1], [\bR_2, \bt_2] \in \mathbb{R}^{3\times 4}$ be their extrinsic matrices.
The ray marching from the camera center $\bo\in\mathbb{R}^3$ through the pixel $\bp\in\mathbb{R}^2$ can be written as $\br_{\bp}(d) = \bR^T(d\bK^{-1}\bar{\bp} - \bt)$, where $d > 0$ indicates the depth along the ray and $\bar{\cdot}$ refers to the homogeneous coordinate.
Denote $\partial\Omega$ as the surface of the scene of interest. The intersection between a ray $\br_{\bp}$ and the scene is $\Phi_{\bp, \Omega} = \{\br_{\bp}(d) | \br_{\bp}(d) \in \partial\Omega \}$. 

The correspondences between the two images $\cI_1$, $\cI_2$ are the set of pixels whose rays intersect at the same, visible 3D surface points:
\begin{align}
\{(\bp_1, \bp_2)~|~\br_{\bp_1}(d_1^*) = \br_{\bp_2}(d_2^*)\}.
\label{eq:ec}
\end{align}
$d_i^* = \arg\min_d \Phi_{\bp_i, \Omega}$ is the depth of the first intersection point between the ray and the scene.
The rest of the intersections $\Phi_{\bp, \Omega} \backslash \br_{\bp}(d^*)$ are not visible in the image due to occlusion. Since the rays of these pixels \emph{explicitly} intersect with one another, we call these pixels \emph{explicit correspondences} (ECs).
\wc{Additionally, the camera origins $\bo_1, \bo_2$ and each pair of ECs are always co-planar. Such a property is called epipolar constraint \citep{hartleymultiple}.}

The goal of correspondence estimation is to identify these ECs from 2D images. Since the appearance of a 3D point may vary with respect to viewpoint due to \eg, illumination effects, \wc{various robust correspondence estimation algorithms $f$ have been proposed~\citep{sift, surf, daisy, superpoint}}. 
While impressive results have been achieved \cite{sift,ranftl2018deep,superpoint,superglue}, these approaches are still limited to scenarios where a large portion of the scene is co-visible.
If the viewpoints change drastically and the observed scenes barely overlap, these methods fail catastrophically\slwang{~\citep{superglue, yang2019extreme}, limiting their applicability in practice.}





\subsection{Bundle Adjustment (BA)}
\label{sec:sfm}

\slwang{Once the explicit correspondences %
are established, we can jointly reason about the camera poses and the 3D position of the correspondences through a procedure called bundle adjustment (BA). BA, however, requires an initialization. We thus estimate the initial relative poses between the selected cameras pairs through the eight-point algorithm and essential matrix decomposition~\citep{longuet1981computer,hartleymultiple}. Once relative camera poses are recovered, we can perform triangulation to recover the 3D scene points from each pair of ECs. 
}
If there are more than 2 images, one can incrementally register them to the existing initial reconstruction or jointly reconstruct them. We refer the readers to \cite{schonberger2016structure} for more details.




Since the estimated ECs contain noise, the initial estimation of 3D points and camera poses are imperfect --- the projection of the triangulated points will not align with their original 2D observations (\ie ECs).
To avoid getting stuck in local, sub-optimal solutions, \sfm
seek to refine the camera poses and the co-visible 3D point locations \slwang{through a joint least-square optimization procedure.}
In particular, we minimize the distance between the reprojected point and observed ECs $\bp_i^j$ for every image $i$ 
in which the 3D point $\bX^j$ is visible:
\begin{align}
\min_{\bR_i, \bt_i, \bX^j} \sum_{i} \sum_{j}~\lVert \bp_i^j - \pi_{\bK_i}(\bR_i\bX^j+\bt_i) \rVert^2.
\label{eq:classic-ba}
\end{align}
\slwang{Efficient least-square solvers, such as Gauss-Newton and Levenberg–Marquardt algorithms are often exploited to tackle the BA algorithms. Minimizing this objective function also has a probabilistic interpretation: it is shown to be equivalent to the Maximum Likelihood Estimation (MLE) under Gaussian observation noise~\citep{agarwal2010bundle}.}
While BA is shown to be very powerful in practice, it heavily relies on ECs to constrain the 3D points. %
If the input images barely overlap and only a few scene points are co-visible, BA may not be able to refine the estimations effectively.


\begin{figure*}
\centering
\includegraphics[trim={0, 11.8cm, 0, 0cm},clip,width=0.95\linewidth]{figs/vc-pipeline.pdf}
\caption{\textbf{Pipeline.} We first predict the 3D shape and pose of the basketball player from the left image. Then we cast a ray and record all the points it hits, \ie the belly button and his back. While the two images barely overlap, the right image does observe the back of player. We can thus tell that the rays of the two pixels intersect at 3D and are virtual correspondences.}
\label{fig:vc-pipeline}
\vspace{-4mm}
\end{figure*}























==> checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{Please see the limitations section~\ref{subsec:limitation}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
   \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{We have included the instructions needed to reproduce the main experimental results in the main paper and in the supplemental material. We will release the code and data upon paper acceptance.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Please see the supplementary material.}
   \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Please see the supplementary material.}
   \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Please see the supplementary material.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{Please see the supplementary material.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{Most of the data we use is from existing public datasets. The new assets are the ground-truth camera trajectories we generated for the curated MC dataset, as well as the 6 MC video snippets we recorded ourselves. We will release them upon paper acceptance.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{We cite and follow the licensing of the public datasets.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{Please see the supplementary material for more details. The data we use is either in the public domain or permitted to release by the participants for research purposes. To the best of our knowledge, the data we are using does not contain offensive content.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> intro.tex <==
\section{Introduction}
\label{sec:intro}

\vspace{-0.05cm}
\begin{quote}
\footnotesize{
``\emph{The closer you look, the less you see.}"}\\[3pt]
\scriptsize{\rightline{--- J. Daniel Atlas, Now You See Me\hspace{1.2cm}}
}
\end{quote}
\vspace{-0.15cm}

Structure from motion (\sfm) aims to recover the 
{geometric structure} of a scene and the spatial layout of the cameras from a set of (unordered) images~\citep{beardsley19963d,fitzgibbon1998automatic,torr1999feature,triggs1999bundle,pollefeys2004visual,snavely2006photo,agarwal2011building}. 
The main idea is to leverage motion parallax to infer 3D geometry \citep{hartleymultiple,ma2012invitation} --- move a camera and observe how
{the same \emph{visible} \joycey{component} of a static scene moves in the projected images accordingly.}
The accuracy of \sfm systems depends on finding good correspondences --- a set of points in one image which can be identified as the same points in another image~\citep{hartleymultiple}. 
The underlying assumption is that the same 3D point in the scene is visible across at least two images~\cite{agarwal2011building}. 
However, the co-visiblity assumption is not always satisfied in practice.
For example, we might want to recover the 3D structure of our favorite movies (Fig.~\ref{fig:teaser} bottom left) or our favorite player's clutch shooting moments (Fig.~\ref{fig:teaser} top left). 
In these settings, %
we might only have access to images with very \joycey{few} co-visible \joycey{3D points, rendering conventional \sfm systems inapplicable}.%

While machines are limited by such constraints, humans are not. %
Consider Fig.~\ref{fig:teaser}. Each pair of images captures the same scene from opposite views. 
Despite such a huge variation in viewpoints, we \joycey{as humans} can still identify where the two photographers were with respect to the scene. 
We can additionally utilize visual cues from the two views to build a coherent, holistic mental view of the 3D world with ease. 
\joycey{Such a remarkable capability comes from our prior knowledge of the underlying geometry, \cbd{which helps us match pixels between images even if their exact correspondences are occluded or invisible in the other image.}}
{ For instance, we know what the front and back of a human body should look like}. %
Therefore, if we see a human face in one image and a back of head on the other, 
we can easily associate them and infer that the two cameras are roughly 180 degrees apart. 




This work aims to equip \sfm systems with similar capabilities and significantly expand their applicable domains to sparse, non-overlapping viewpoints.
{Consider again the non-overlapping image pair in the bottom left of Fig.~\ref{fig:teaser}. 
Conventional \sfm system fails here because it requires the matched pixels to represent the same, 
co-visible 3D point in order to establish two intersecting camera rays shooting into the scene. 
However, if the system has prior knowledge about human shape, 
it will know that a ray shooting through the human back in the left image will intersect with the chest region on its way out. Better yet, the intersecting chest pixel can be observed in the right image. Thus, we can find a pair of pixels that also correspond to two intersecting camera rays, except they depict different 3D points in the scene.} \shenlong{I feel this paragraph could be merged to para 2 and next para; contents are redudant.}







With this motivation in mind, we present \emph{virtual correspondences} (VCs), a generalization of existing {explicit correspondences} (ECs).
VCs are a pair of pixels from two images where their associated camera rays intersect in 3D (see Fig.~\ref{fig:vc-bunny}). %
Similar to ECs, VCs also %
conform to epipolar geometry. 
However, unlike ECs, 
VCs do not require pixels to describe the same, co-visible 3D points, thus, they are more flexible. 
VCs can have completely different semantics and appearances; they can also be established across images with extreme poses. 
We integrate VCs \joycey{with learned shape priors} into the classic bundle adjustment algorithm 
and propose a generalized \sfm framework, exploiting both explicit and virtual correspondences. \joyce{It is still confusing to me how we talk about ECs and VCs separately since VCs are just a superset}
Compared to conventional \sfm, our generalized framework can be applied to a much more comprehensive range of scenarios, 
including extreme cases such as two-view \sfm with 180 degrees viewpoint differences, as shown in Fig.~\ref{fig:teaser}.  

We demonstrate the effectiveness of our approach on the CMU Panoptic dataset \cite{Joo_2015_ICCV,Joo_2017_TPAMI}, 
the Mannequin Challenge dataset \cite{li2019learning}, and multiple challenging in-the-wild images. 
Our method significantly outperforms previous state-of-the-art \sfm systems 
and other baselines in challenging scenarios \cbd{and is comparable in the conventional, densely overlapped setup}. 
Although we mainly conduct our experiments on human datasets in this paper, we believe our generalized \sfm framework can be applied to a wide range of scenes and objects
such as cars, animals, rooms, and buildings.   















\begin{figure}
\includegraphics[trim={0, 7.2cm, 0, 0},clip, width=\linewidth]{figs/teaser-new-no-bg.pdf}
\caption{\textbf{Can you tell where the cameras are?} 
\slwang{We present a generalized \sfm algorithm that can reconstruct the 3D human shapes and recovers the camera poses even if the inputs have no overlap.
}}
\vspace{-4mm}
\label{fig:teaser}
\end{figure}















































































==> method.tex <==
















\subsection{Generalized Bundle Adjustment} 
\label{sec:generalized-ba}
{With the established virtual correspondences, the next step is to jointly reason the camera poses as well as the 3D scene geometry. Similar to classic \sfm, we initialize the poses using RANSAC with the eight-point algorithm~\citep{hartleymultiple} in the loop. But instead of employing ECs, we use VCs.


We first recover the 3D locations of the VCs. The triangulation approach used for ECs is not applicable since VCs could correspond to different surface points, as shown in Fig.~\ref{fig:vc-bunny}. We thus leverage the initial shape estimation to compute the ray-surface intersection and record the first hits for each image. The 3D points are then registered into the global coordinate system using the initial camera poses.}


{Since the estimated structure and poses depend heavily on the predicted shape priors, they may be noisy. We further refine the estimates by minimizing the distance between reprojected points and VCs. Unlike traditional \sfm, VCs may not share the same visible surface points. Nevertheless, the rays connecting the camera center and each 3D point are co-planar. We can thus re-write one VC point as a function of the other with two free parameters $\alpha^j$ and $\beta^j$:
\begin{align}
\bX^j_2 = \bX^j_1 + \alpha^j \cdot (\bX^j_1 - \bo_1) + \beta^j \cdot 
(\bo_2 - \bo_1), \text{\ \ where \ \ } \forall i,  \bo_i = -\bR_i^T \bt_i, \alpha^j \geq 0; \beta^j \geq 0
\end{align}
Intuitively, $\alpha^j$ and $\beta^j$ can be treated as the ``thickness'' of the intersecting points to the surface along the ray direction. VCs reduce to ECs when both parameters equal 0. 
Thus, one could jointly minimize the following generalized bundle adjustment problem. 
\begin{align}
\min_{\bR_i, \bt_i, \bX^j_1, \alpha^j, \beta^j} & \sum_{i} \sum_{j}~\lVert \bp_{i, 1}^j - \pi_{\bK_i}(\bR_i\bX^j_1+\bt_i) \rVert^2 + \lVert \bp_{i, 2}^j - \pi_{\bK_i}(\bR_i\bX_2^j + \bt_i) \rVert^2.
\label{eq:generalized-ba}
\end{align}
where $\bp_{i, 1}^j, \bp_{i, 2}^j$ are observed VC pairs, for images $i$ in which $\bX_1^j, \bX_2^j$ are visible. 
By minimizing the objective, we are essentially adjusting a bundle of \emph{line segments pairs}, rather than a set of \emph{3D points} as in classic \sfm. We use L-BFGS~\cite{nocedal1980updating} %
to solve this non-linear least square problem. Note that ECs are a special case of VCs where the tuple of line segments are reduced to 3D points. Such formulation allows bundle adjustment to include both ECs and VCs. 
}








































\paragraph{Relationship to traditional \sfm:}
VCs can be combined with classic correspondences to improve the overall robustness and performance of the 3D reconstruction system. When the images barely overlap and little traditional correspondences are available, the system can rely on VCs to recover the world and camera geometry. When the images do overlap, VCs can serve as additional visual cues and regularizers. VCs significantly expand the applicable setting of existing SfM systems.


















==> old_vc.tex <==
\subsection{Old Virtual Correspondences}


As we have alluded in Sec. \ref{sec:single-image-3d}

For simplicity, we start with a setting where there are only two cameras, but the notion can be directly applied to $n$ camera scenario.
Let $\bK_1, \bK_2$ be the camera intrinsics, and $[\bR_1, \bt_1], [\bR_2, \bt_2]$ be the extrinsic matrices. We can parameterize the ray shooting from the camera origin through the pixel $\bp = (u, v)$ as 
\begin{align*} 
\br_{\bp,c}(d) = \bR_c^T(\bK_c^{-1}\begin{pmatrix}u_c\\v_c\\d_c\end{pmatrix} - \bt_c),~~d > 0,
\end{align*}
where $d_c$ represents the distance to the camera $c$.

To estimate the depth of the pixel, one can compute the intersection between the ray and the surface of the scene $\Omega$:
\begin{align*}
d_{\bp,c} = \arg\min~\br_{\bp,c}(d),~~~~\text{s.t.}~~\br_{\bp,c}(d) \in \Omega.
\end{align*}

Let $\bp_1, \bp_2$ be the pixels of the two images respectively. %
The two pixels are defined as correspondence if they are the projection of the same 3D point. To be more formal, 
\begin{align*}
\cC = \{(\bp_1, \bp_2)~|~\br_{\bp_1,1}(d_{\bp_1,1}) = \br_{\bp_2,2}(d_{\bp_2,2})\}
\end{align*}

In this paper, we relax the constraint. We define the two pixels as  correspondences so long as the two rays intersect. We do not care if the intersection point is visible - the rays can intersect behind the occlusion.
\begin{align*}
\cC = \{(\bp_1, \bp_2)~|~\br_{\bp_1,1}(d_{1}) = \br_{\bp_2,2}(d_{2})\}
\end{align*}

The next question is: \emph{how do we know the rays will intersect if we are not aware of the camera poses and there is occlusion?}


If we know the shape and pose of an object, one trivially compute all the intersection points between the ray and its surface.
\begin{align*}
\cH_{\bp,c} = \{d ~|~\br_{\bp,c}(d) \in \cM\}.
\end{align*}

==> related.tex <==
\section{Related Work}
\label{sec:related}

\paragraph{Structure from motion (\sfm):}
Given a set of unordered images depicting the same scene, structure from motion algorithms attempt to recover both the camera poses (motion) and the 3D geometry of the scene (structure). An \sfm framework usually represents images as sets of keypoints, establishes explicit correspondences among them, and performs epipoloar geometry-based pose estimation~\citep{beardsley19963d,fitzgibbon1998automatic,torr1999feature,triggs1999bundle,pollefeys2004visual,snavely2006photo,agarwal2011building,schonberger2016structure}. To jointly refine poses and the 3D structure, bundle adjustment (BA)~\citep{szeliski1994recovering,cooper1996theory,triggs1999bundle} is then applied. While there has been a surge of interest in exploiting photometric error as the BA objective lately~\citep{photometricba,tang2018ba,barf}, 
most methods still follow the \emph{gold standard} and minimize the geometric reprojection error~\citep{hartleymultiple,torr1999feature}. Our approach is a generalization of existing \sfm methods with virtual correspondences. While semantic \sfm~\citep{bao2011semantic} also leverages semantic cues, we handle much more challenging wide-baseline image pairs.














\begin{figure}[t]
\centering
\includegraphics[trim={0, 6.8cm, 0, 0cm},clip,width=0.9\linewidth]{figs/bunny-new.pdf}
\caption{\textbf{Explicit correspondences vs virtual correspondences.} \slwang{Explicit correspondences' camera rays intersect at the same visible 3D surface point. Virtual correspondences' ray also intersect, but do not require to be co-visible across views.}}
\label{fig:vc-bunny}
\vspace{-4mm}
\end{figure}





\paragraph{Correspondences: }
Correspondences are fundamental in computer vision to help
recover the relative camera parameters~\citep{longuet1981computer}, estimate the motion of the world~\citep{horn1981determining}, and reconstruct the 3D scene geometry~\citep{hartleymultiple}.
Conventional feature correspondences focus on identifying image pixels that share similar appearance using classical~\citep{sift,surf,daisy,brisk,orb} or learned~\citep{wang2016global,autoscaler,superpoint,superglue,wang2019learning,wang2020caps} feature extractors. On the other hand, semantic correspondences~\citep{siftflow,daisyflow,proposalflow,flowweb,zhou2016learning,choy2016universal,kim2017fcss,scnet,scops} find keypoint pairs that are semantically similar. 
In addition, \citep{raposo2016pi} creates plane-level correspondences and \citep{cai2020messytable} establishes correspondences between objects. 
Different from most existing correspondences 
that seek to represent the same underlying co-visible 3D points explicitly, 
our proposed virtual correspondences do not necessarily share similar appearances or semantics, 
so long as their associated camera rays intersect in 3D. 




\paragraph{Extreme relative pose estimation: } %
Several works have tackled image matching with extreme baselines. \citep{cai2021extreme} constructs a deep dense correlation volume for each image pair to estimate relative 3D rotation. \citep{yang2019extreme,yang2020extreme} learn scene completion on input RGB-D scans.%
\citep{xu2021widebaseline} treats the center of mass for each human as a keypoint and establishes correspondences with human re-identification. \citep{qian2020associative3d} predicts the pose and volumetric representation for each object in an indoor room and stitches them with restrictive assumptions on camera and scene configurations. Different from these approaches, our method integrates learned parametric 3D shape priors~\cite{SMPL:2015,SMPL-X:2019} into a traditional \sfm pipepline, which (1) naturally extends to multi-view settings, (2) obtains accurate poses through continuous optimization with geometric constraints, and (3) generalizes well to unknown scenes as pose estimation is an inference process that does not require training. Although~\citep{dong2020imocap} also jointly estimates human shape parameters with human poses, their application domain is in human motion capture while we focus on general relative pose estimation between images. In addition, our method can be extended with other parametric models such as animals~\citep{SMAL}, cars~\citep{engelmann2017samp}, furniture~\citep{gao2019sdm} and generic 3D shapes~\citep{lin2020sdf, zhang2018learning}. %











==> vc.tex <==



\begin{figure*}
\centering

\setlength\tabcolsep{4pt}
\def\arraystretch{0.3}
\setlength{\tabcolsep}{0.5pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{cccc}
\raisebox{1.5cm}{\multirow{2}{*}{\includegraphics[height=3.2cm,width=0.02\linewidth,trim={1mm, 0cm 2mm 0cm},clip]{figs/color_bar.pdf}}}
&\includegraphics[width=0.31\linewidth]{figs/qual-correspondence/0a312f741fdf5d89-two_teachers_8_30_shorter_015318-sg.pdf}
&\includegraphics[width=0.31\linewidth]{figs/qual-correspondence/0a312f741fdf5d89-two_teachers_8_30_shorter_015318-loftr.pdf}
&\includegraphics[width=0.31\linewidth]{figs/qual-correspondence/0a312f741fdf5d89-two_teachers_8_30_shorter_015318-ours.pdf}\\
&\includegraphics[width=0.31\linewidth]{figs/qual-correspondence/0a312f741fdf5d89-two_teachers_8_30_shorter_015318-sg.pdf}
&\includegraphics[width=0.31\linewidth]{figs/qual-correspondence/0a312f741fdf5d89-two_teachers_8_30_shorter_015318-loftr.pdf}
&\includegraphics[width=0.31\linewidth]{figs/qual-correspondence/0a312f741fdf5d89-two_teachers_8_30_shorter_015318-ours.pdf}\\
&\footnotesize{(a) SuperGlue} & \footnotesize{(b) LoFTR} & \footnotesize{(c) Ours}
\end{tabular}
}
\caption{\textbf{Qualitative comparison.} \weichiu{find new figures for second row}}
\label{fig:vc-qual-comp}
\end{figure*}

\section{Generalized Structure {from} Motion}
\label{sec:method}

Our aim is to develop a generic \sfm algorithm that is capable of recovering camera poses as well as scene geometry whether the input images overlap or not. 
Towards this goal, we present \emph{virtual correspondences} (VCs), a generalization of existing ECs. 
VCs respect epipolar geometry and can be found across images that do not overlap, allowing us to construct geometric relationships even when no ECs are available. 
In this section, we first formally define VCs. Then we describe their geometric properties as well as how to find them efficiently. Next, we show that VCs can be integrated into the existing \sfm pipeline, resulting in a generic, robust \sfm system that can handle various scenarios. Finally, we discuss our design choices and their relationship to related work.








\subsection{Virtual Correspondences}
\label{sec:vc}
As we allude to in previous sections, virtual correspondences is a set of pixels whose camera rays intersect in 3D:
\begin{align}
\{(\bp_1, \bp_2)~|~\br_{\bp_1}(d_1) = \br_{\bp_2}(d_2)\}.
\label{eq:vc}
\end{align}
There is no constraint on where the intersection {between each camera ray and the surface} should happen. The rays can intersect at (i) co-visible surface points, (ii) surface points that are only visible in one image, or even (iii) non-surface points.
In the first scenario, the intersecting point can be written as $\br_{\bp_1}(d_1^*) = \br_{\bp_2}(d_2^*)$. Eq. \ref{eq:vc} thus becomes equivalent to Eq. \ref{eq:ec} and VCs reduce to ECs. 
In the second and the third scenario, the visible surface points of VCs are different. VCs %
can thus have different appearances and semantics, and even describe completely different parts of the scene. 
The VCs in Fig. \ref{fig:vc-bunny} correspond to the second scenario. 
The pixels in the left image observe the leg while their VCs in the right see the back.




One key property of VCs is that they conform to epipolar constraints --- the two intersecting rays form an epipolar plane on which the VCs and camera origins lie.
This allows us to exploit classic geometric algorithms to establish connections among non-overlapping images, greatly expanding the applicable domains of existing 3D algorithms.
For instance, we cannot employ the eight-point algorithm~\cite{longuet1981computer} for non-overlapping images in the past, since no ECs exist. VCs, however, are more flexible than ECs and are not restricted to describing the same co-visible surface points. We can thus estimate VCs among the images and then solve for the fundamental matrix. 
We refer the readers to supp. material for more discussion on VCs and epipolar geometry.


\paragraph{Estimating virtual correspondences: } While VCs are powerful, 
estimating them purely from 2D images is far from trivial. VCs may have completely different appearances and semantics, prohibiting us from employing similar approaches as explicit correspondence estimation.
In this work, inspired by how humans leverage prior knowledge to perform 3D reasoning, we propose {one approach} to exploit shape priors for virtual correspondence estimation. 
{Our approach works as follows.} %
Given {all 2D images, we first make an initial prediction of the 3D shape and pose for each image.}
Then, we cast a ray through {each} pixel and record all the surface points the ray hits. Finally, if any other images observe {those surface points based on the initial shape and pose predictions,}
we {say} the two pixels intersecting in 3D are VCs. Fig. \ref{fig:vc-pipeline} illustrates the process. %

We implement both the monocular 3D reconstruction model and the 2D-3D association model as neural networks. Specifically, we use HMR-Net \cite{kanazawa2018end} to predict the 3D human mesh and pose in each image, and exploit DensePose \cite{guler2018densepose} to estimate the 3D-to-2D mapping.
We note that while we focus on humans, our formulation is generic and can be applied to other {objects or scenes where parametric 3D models could be constructed, such as vehicles, CAD models, buildings and animals.} %

